Educational Question Generation of Children Storybooks via Question Type Distribution Learning and Event-Centric Summarization

Generating educational questions of fairytales or storybooks is vital for improving children's literacy ability. However, it is challenging to generate questions that capture the interesting aspects of a fairytale story with educational meaningfulness. In this paper, we propose a novel question generation method that first learns the question type distribution of an input story paragraph, and then summarizes salient events which can be used to generate high-cognitive-demand questions. To train the event-centric summarizer, we finetune a pre-trained transformer-based sequence-to-sequence model using silver samples composed by educational question-answer pairs. On a newly proposed educational question answering dataset FairytaleQA, we show good performance of our method on both automatic and human evaluation metrics. Our work indicates the necessity of decomposing question type distribution learning and event-centric summary generation for educational question generation.

==> sections/method_old.tex <==
\section{Method}

\begin{figure*}
    \includegraphics[width=\textwidth]{figures/overview}
    \caption{The overview of fairytale question generation system.}
    \label{overview}
\end{figure*}

The overview of our fairytale question generation system is shown in Figure \ref{overview},
which contains two parts: fairytale summarization and question generation.

\subsection{Fairytale Summarization}

\subsubsection{Discourse-aware Graph Construction}

We construct a discourse-aware token-level graph to encode fairy tales,
where we model dependency relations both within and among discourses.
In particular, given an input fairytale section, we first segment it into 
elementary discourse units (EDUs) \cite{wang-etal-2018-toward},
and then parse the dependency relations among EDUs \cite{li-etal-2014-text}.
For each EDU, we construct a subgraph using dependency parsing \footnote{\url{https://spacy.io/api/dependencyparser}}. 
Afterwards, we connect the root node of each EDU via the dependency relations of each EDU. 
An example is shown in Figure \ref{overview}.

\subsubsection{GNN Encoder}

With our discourse-aware graph construction, we can obtain a token-level graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$,
where each node $v_i \in \mathcal{V}$ denotes a token and each edge $e_{ij} \in \mathcal{E}$ 
denotes the dependency relation between tokens. 

We employ graph attention networks (GAT) \cite{gat} 
to encode the graph, and obtain representations of each node. In particular, consider the representations 
of each node at layer $l$ as $\boldsymbol{h}=\{ \overrightarrow{h}_1, \overrightarrow{h}_2, \ldots,
\overrightarrow{h}_N \}$, we would like to calculate the representations 
of each node at layer $l+1$ as $\boldsymbol{h}'=\{ \overrightarrow{h}'_1, \overrightarrow{h}'_2, \ldots,
\overrightarrow{h}'_N \}$. When $l=0$, $\boldsymbol{h}$ is the input embeddings of each token 
$\boldsymbol{x} = \{\overrightarrow{x}_1, \overrightarrow{x}_2, \ldots, \overrightarrow{x}_N \}$.

The $\boldsymbol{h}'$ is obtained through a multi-head attention mechanism:

\begin{equation*}
    \overrightarrow{h}'_i = \text{concat}_{k=1}^K \sigma(\sum_{j \in \mathcal{N}_i} \alpha_{ij}^k \boldsymbol{W}^k \overrightarrow{h}_j),
\end{equation*}

\noindent where $\text{concat}$ denotes the concatenation operator, $K$ is the total number of heads,
$\mathcal{N}_i$ denotes the neighborhoods of node $i$, $\boldsymbol{W}^k$ is a learnable matrix, 
$\sigma$ denotes a nonlinear transformation, $\alpha_{ij}$ denotes the attention of node $j$ to node $i$:

\begin{equation*}
    \alpha_{ij} = \frac{\exp (LeakyReLU (\boldsymbol{a}^T [\boldsymbol{W}\overrightarrow{h}_i || \boldsymbol{W}\overrightarrow{h}_j] ))}{\sum_{k \in \mathcal{N}_i} \exp (LeakyReLU (\boldsymbol{a}^T [\boldsymbol{W}\overrightarrow{h}_i || \boldsymbol{W}\overrightarrow{h}_k] ))}.
\end{equation*}

% We use graph convolution network (GCN) \cite{kipf2016semi} to encode our discourse-aware token-level graph. In particular,
% considering token embeddings $\boldsymbol{x}_1, \boldsymbol{x}_2, \ldots, \boldsymbol{x}_n$,

% \begin{equation*}
%     f(\boldsymbol{x}_i) = \boldsymbol{U}f(\boldsymbol{\varLambda})\boldsymbol{U}^T \boldsymbol{x}_i
% \end{equation*}

% \begin{equation*}
%     \boldsymbol{H}^{(l)} = \sigma( \Tilde{D}^{-\frac{1}{2}}\Tilde{A}\Tilde{D}^{-\frac{1}{2}}\boldsymbol{H}^{(l-1)}\boldsymbol{W}^{(l-1)}),
% \end{equation*}

% \noindent where $\Tilde{A}=A+I_n$, $A$ is the adjacent matrix, $D$ is the degree matrix, $\Tilde{D}_{ii}=\sum_j{\Tilde{A}_{ij}}$, $\boldsymbol{W}$ is a layer-wise learnable matrix, $\boldsymbol{H}^{(l)}$ is node representations at layer $l$, and the input layer $\boldsymbol{H}^{(0)}=[\boldsymbol{x}_1, \boldsymbol{x}_2, \ldots, \boldsymbol{x}_n]$.

% \textbf{When it comes to the directed graphs, few GNN methods such as GGNN, GAT still work.}

\subsubsection{Sequential Decoding}

We use graph to sequence decoding method to decode our output summarization \cite{2106.06090}. 
In particular, with the node embeddings obtained via GAT, we can decode the output summary sequence sequentially. 
We use LSTM as the decoding module. The following four common techniques are from \cite{2106.06090}.

\paragraph{Attention}

At each decoding step $t$, we first compute an attention vector indicating the distribution over some words:

\begin{align*}
    e_i^t &= f(\overrightarrow{h}_i, \overrightarrow{s}_t),\\
    \overrightarrow{\alpha}^t &= softmax(\overrightarrow{e}^t)
\end{align*}

\noindent where $\overrightarrow{s}_t$ denotes the decoding state,
$\overrightarrow{h}_i$ is the encoding hidden state. The context vector then is:

\begin{equation*}
    \overrightarrow{h}_t^* = \sum_i \alpha_i^t \overrightarrow{h}_i
\end{equation*}

\paragraph{Copy mechanism}

At each decoding step, we calculate the probability of whether copying a word from the input sequence by sampling attentions or generate a token from the output vocabulary:

\begin{equation*}
    p_{copy} = \sigma(\boldsymbol{w}_{h^*}\boldsymbol{h}_t^* + 
    \boldsymbol{w}_{s^T}\boldsymbol{s}_t+\boldsymbol{w}_x\boldsymbol{x}_t + b_{ptr})
\end{equation*}

\paragraph{Coverage mechanism}

Coverage mechanism is utilized to encourage to use all vocabulary in the input sequence.

\begin{equation*}
    \boldsymbol{c}^t = \sum_{t'=0}^{t-1}\boldsymbol{a}^{t'},
\end{equation*}

Then the new attention is obtained by:

\begin{equation*}
    e_i^t = f(\boldsymbol{h}_i, \boldsymbol{s}_t, c_i^t)
\end{equation*}

Finally, a coverage loss is used to avoid generating repeated text:

\begin{equation*}
    covloss_t = \sum_i \min(a_i^t, c_i^t).
\end{equation*}

\paragraph{Scheduled sampling.}



\subsection{Transformer-based Question Generation}

We fine-tune a BART model \cite{lewis-etal-2020-bart} to generate questions based on the summarization 
obtained from the previous section.
